Implicit Discourse Relation Classification For Nigerian Pidgin

Despite attempts to make Large Language Models multi-lingual, many of the world's languages are still severely under-resourced. This widens the performance gap between NLP and AI applications aimed at well-financed, and those aimed at less-resourced languages. In this paper, we focus on Nigerian Pidgin (NP), which is spoken by nearly 100 million people, but has comparatively very few NLP resources and corpora. We address the task of Implicit Discourse Relation Classification (IDRC) and systematically compare an approach translating NP data to English and then using a well-resourced IDRC tool and back-projecting the labels versus creating a synthetic discourse corpus for NP, in which we translate PDTB and project PDTB labels, and then train an NP IDR classifier. The latter approach of learning a "native" NP classifier outperforms our baseline by 13.27\% and 33.98\% in f$_{1}$ score for 4-way and 11-way classification, respectively.

==> sections/abltationStudy.tex <==
\section{Ablation Study} % think this could use a different title, something like "extended results & discussion" (but then a more flowy sounding equivalent)
\label{sec:ablation}

This section discusses the effects of the different projection methods for corpus creation (alignment-based and relation-based) and fine-tuning methods for the word alignment tools (PFT and CAT). All results for all set-ups are included in Table \ref{tab:ablation}. 
%We hypothesize that fine-tuning state-of-art aligner AweSoME using real parallel datasets provided by \cite{pcm_paper_baseline, lin2023low} could enhance the aligner's - AweSoME+PFT- understanding of the relationship between parallel English and NP, and this has been stated in the results as Naija model with T5 large trained using CaFT on dataset generated with AweSoME+PFT model, results in the best f$_{1}$. % think this has already been said in the previous section, right?
As mentioned in Section \ref{sec:intro}, we expect the alignment-based method to result in slightly noisier data compared to the relation-based method, as words might be missing from arguments due to alignment errors. However, we expect the translation quality for the alignment-based method to be slightly better than for the relation-based method, as context is taken into account during translation. 
The effect of this can be seen by comparing the results of \textbf{Naija model with CAFT} and \textbf{Naija model from scratch} in the top half of the table (under \textbf{RELATION-BASED}) with the corresponding rows in the bottom half of the table (under \textbf{ALIGNMENT-BASED}). %, for the . CAFT or the Scratch Naijamodel training between the dataset of the \textbf{RELATION-BASED} compared to that of the \textbf{ALIGNMENT-BASED}, in which \textbf{RELATION-BASED} dataset with CaFT results in the state-of-art resulrs.  
%From the results in \ref{tab:ablation}, we can see that the \textbf{SimAlign} for the 4-way classification is based on 46.1\%, which is 13.27\% more than the Zeroshot NP. Moreover, it can be stated that for most of the cases, when using the T5-Large variant of the models with CaFT for both the \textbf{RELATION-BASED} and \textbf{ALIGNMENT-BASED}.

%We suspect that the large models are more prone to over-fitting than their base versions, due to their larger number of parameters. Any noise introduced in the training data might thus be affecting the larger models more. Indeed, we see that the performance gain, especially when looking at 11-way f$_{1}$, comparing \textbf{Naija model from scratch} with \textbf{Naija model with CAFT}, is larger for the large model, as this is a continuation of an English-trained model, leading to more robustness and presumably less over-fitting. % PB 10-06-2024: hmm, I'm not too sure about this over-fitting argument, actually. First, we should carefully say that it's a hypothesis, and we didn't explicitly look for particular signs of over-fitting. But, perhaps more importantly; DiscoPrompt is trained on the English PDTB, right? With the CAFT setup, we continue fine-tuning it, on NP versions of (again) PDTB relations. So in a way, the model has seen the same relations twice, just in different languages. What does this mean for the whole over-fitting idea? If training on the same relations twice results in better scores, doesn't that mean that over-fitting is actually beneficial, in a way?

%Moreover, we hypothesize in \ref{sec:intro}, for both the \textbf{ALIGNMENT-BASED} as well as the \textbf{RELATION-BASED} that when training DiscoPrompt on NP from scratch, the larger variants would over-fit to the training dataset, as our dataset is automatically generated, and this cleary shows the importance of CaFT in which the IDRC is able to transfer the information it posses about the relation classification with our generated dataset and resulting in the state-of-art results.

Because we obtain the highest scores using the large models, we conclude that for our use case, translating arguments in isolation (\textbf{RELATION-BASED}), thereby risking losing some context, is better than preserving context during translation and relying on word alignment to correctly retrieve all tokens that make up the arguments.
With regard to the question of using a zero-shot set-up on NP (either directly or on a translated version of the input text), or training a dedicated NP model, Table \ref{tab:4_setups} already illustrated that it is best to train a dedicated NP model, that uses an English model as basis and further fine-tunes this on synthetic NP discourse relations. In Table \ref{tab:ablation}, we can furthermore see that PFT always improves performance for AWESoME; on the contrary, CAT usually decreases performance for SimAlign. In line with earlier work, though, both neural aligners outperform Giza-py overall.

% \textcolor{blue}{we are providing a confusion matrix for the IDRC using the Naijamodel Caft with AweSoME+PFT} \textcolor{red}{@Muhammed; thanks for including the confusion tables. Two main things from this are missing though, for them to be informative: 1) could you replace the first column entries (under ``class'') with their actual label? (i.e. comparison, contingency, expansion, temporal for 4-way, and the concession etc. ones for 11-way? Just having numbers in there doesn't mean anything to anyone. And 2) the number of support cases for each class/label, as an additional column (to the right). We can then a) see if some particularly low score is perhaps not very reliable, because it's based on a very small nr of support cases, and b) if that number is perhaps very different from the distribution in the training data (this we have in Figure 4 in appendix A).}
\input{tables/confusionMatrix/AweSoMEPFT_11Way}
% \input{tables/confusionMatrix/AweSoMEPFT_4Way}



==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\textcolor{red}{this section discusses the results we got }

==> sections/futurework.tex <==
\section{Futurework}
\label{sec:futurework}
Future work will focus on expanding the NP PDTB to include more diverse discourse relations and larger datasets to enhance model training and evaluation. We aim to explore additional fine-tuning techniques and advanced annotation projection methods to further reduce noise and improve model performance. Investigating the applicability of our approaches to other low-resource languages will also be a priority, potentially creating a framework for IDRC across various linguistic contexts. Furthermore, integrating more sophisticated language models and cross-lingual transfer learning strategies may yield even better results, contributing to the broader field of computational linguistics.



==> sections/introbefore23may.tex <==
\section{Introduction}
\label{sec:intro}

In this  research we  addressing  the development of an Implicit Discourse Relation Classification (IDRC) system for Nigerian Pidgin (NP). A primary challenge for this task  is the absence of a Nigerian Pidgin Penn Discourse Treebank (NP PDTB), essential tool for training IDRC. Our study explores a various  strategies to overcome bridge this  barrier, by testing four setups to handle the IDRC of NP. The first setup  ZERO SHOT PIDGIN involves employing zero-shot learning with state-of-the-art English models \cite{chan2023discoprompt}, directly on NP data. The second strategy,  ZERO-SHOT TRANSLATION, involves translating the NP test set into English and then applying English IDRC models \cite{chan2023discoprompt} to these translations. Our third and fourth approaches delve deeper into the creation of an NP PDTB, utilizing machine translation and alignment techniques to annotate NP discourse automatically. The NAIJA MODEL setups trains DiscoPrompt model exclusively on this newly created NP PDTB, while the Continual Adaptive Finetuning (CaFT) approach uses the NP PDTB to fine-tune a model initially trained in English \cite{chan2023discoprompt}. As both Naija Model and CaFT setups employs finetuing on NP PDTB we have to address the propagated errors from machine translation and alignment is a significant concern. The creation of the PDTB dataset involves annotation projection which we are going to employ two methodologies the first is the Fulltransfer which involves analysis of the continuous Arguments and then translating those directly and the discontinuous  which involve Alignment centeric method, that is based totally on the alginments. Moreover, to try and handle the propagated we have employed first contextualized aligner modes such as the \cite{dou2021word, sabet2020simalign}  to generate the NP PDTB, besides fine-tuning \cite{dou2021word} on real parallel corpora provided\cite{ pcm_paper_baseline, lin2023low} which called PFT, also crosslingual adaptive training for the simAlgin model  "CaT", in which for the \cite{sabet2020simalign} aligner model we used  the state-of-art NP RoBERTa  \cite{lin2023low}. However as both the parallel data used for the PFT and the \cite{lin2023low} RoBERTa model are trained on religious content which is of other domain dataset comapered to the PDTB and the dataset is limited then the model mayoverfit this dataset and the results not always the best.
And another important piece of information we need is to test which DiscoPrompt Large/ Base will best suit NP IDRC classification, as for the zeroshot and Translation zero shot it makes sense that hte DP Large model is better and there can be overfitting when finetuing the DiscoPrompt Large on the NP-PDTB as due to the noise. By systematically testing these methodologies, this research aims to offer valuable insights into the most effective strategies for implementing IDRC in low-resource settings like Nigerian Pidgin. Which can provide valuable insights for other low-resource languages. In General we CaFT with the dataset from the Fulltrasnfer method will report the state-of-art results as this dataset is less noisy compared to AC dataset and we also hypothesis that DiscoPrompt Large with the AC will overfit the training dataset and the model performance will drop compared to use the BASE variant due to the propagated noise is doubled and the model then will probably memories this noise.

==> sections/methodology.tex <==
\section{System Architecture}
\label{sct:system}

The overall architecture of our system is outlined in Figure \ref{fig:pipeline}. % PB 12-02-2024:  figure needs to be redone.
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth, height=0.6\textheight, keepaspectratio]{images/ACL Pidgin IDRC paper pipeline .drawio (6).png}
    \caption{Paper Pipeline}
    \label{fig:pipeline}
\end{figure*}

The main contribution of this paper is two-fold: First, we generate several variations of an NP corpus of implicit discourse relations. These originate from using different word aligners to project the original, PDTB implicit relations onto the NP translations of the English source text. Second, we experiment with different setups for implicit discourse relation classifications, and evaluate these on the different variations of our NP corpus of implicit relations.
To translate the original English text to NP, we directly use the system proposed by \citet{lin2023low} without any further modifications. The modifications we make to the word alignment and relation classification systems we adopt are detailed in the following sections.

\subsection{Word Alignment}
\label{ssct:alignment}
Our research focuses on the implicit relations from the PDTB (see Section \ref{ssct:relclass} for more details). Since we use the PDTB2 \cite{Prasad08thepenn}, implicit relations are annotated over adjacent sentences. As such, more coarse \textit{sentence} alignment, as opposed to \textit{word} alignment, would suffice, and translating on a sentence-by-sentence basis would automatically give us the aligned sentences. However, when translating sentence-by-sentence, it is not straightforward how to take context into account, and given that we are dealing with \textit{discourse} relations, which, in the case of PDTB2 implicit, by definition, exhibit themselves beyond the sentence level, we opt for translating the entire text first and then finding the sentences, or arguments of the relations, through word alignment. Word alignment is done on the entire text, as the number of sentences for the original English text and the translated NP text is not necessarily identical.
In our setup, we include the following aligners:
\begin{itemize}
    \setlength\itemsep{-0.5em}
    \item Giza-py\footnote{\url{https://github.com/sillsdev/giza-py}}
    \item SimAlign \cite{sabet2020simalign}
    \item AWESoME \cite{dou-neubig-2021-word}
\end{itemize}

Giza-py is a Python implementation of GIZA++ \cite{10.1162/089120103321337421} and cannot be fine-tuned for a particular language, so we use this aligner ``as is''.
Out-of-the-box, SimAlign uses a combination of fastText \cite{10.1162/tacl_a_00051}, multi-lingual BERT \cite{devlin2018bert} and XLM-RoBERTa base \cite{conneau-etal-2020-unsupervised} embeddings. We generate one version of our corpus using the code provided by \citet{sabet2020simalign}. To generate more accurate alignments, we modify SimAlign by applying Cross-lingual Adaptive Training (CAT) to RoBERTa \cite{liu2019roberta}, to adapt it to NP specifically.  
In their recent study, \citet{lin2023low} introduced the CAT method, an advanced approach for tuning LLM for better low-resource natural language understanding, which involves fine-tuning of an English RoBERTa model \cite{liu2019roberta} on collected noun phrases (NPs). Their findings indicate that this fine-tuned model exhibits superior performance in NP sentiment analysis compared to the English variant used in \cite{muhammad2022naijasenti} study. Building on this, our research intends to apply the fine-tuning approach of \cite{lin2023low} to the Simalign model \cite{sabet2020simalign} to create a new set of annotated NPs for PDTB.

%We follow the procedure of \citet{lin2023low}.
% This is then used to generate another version of our NP corpus.

For AWESoME, in addition to an out-of-the-box version of the alignments, we use Parallel fine tuning (PFT) to adapt it to NP. The model proposed by \cite{dou2021word}facilitates the refinement of aligner models using parallel data. In our research, we plan to utilize the parallel corpus as provided by \cite{lin2023low}, and the \cite{pcm_paper_baseline}. Our objective is to fine-tune the aligner model specifically for the English and NP  language pair. Subsequently, this fine-tuned aligner model will be employed to generate a new subset of an annotated NP projected dataset.


Finally, we end up with five different versions of our NP corpus of implicit relations: One for Giza-py, two for the standard and adapted versions of SimAlign, and two for the standard and adapted versions of AWESoME. Since we have no gold standard for the alignments, we cannot calculate an alignment error rate, and while we assume that the SimAlign and AWESoME models adapted to NP will perform better, we have no way of automatically checking this. We thus proceed with these five versions of our NP corpus, and use this for training and evaluation of the implicit relation classifier. It may be tempting to treat classification performance as an extrinsic evaluation of word alignment as well. In other words, if the classification f1-score for the same classifier on the SimAlign+CAT corpus is better than on the SimAlign (without CAT) corpus, one might want to conclude that CAT improves alignment results. We argue, however, that this may instead indicate that a certain and consistent error in alignment is picked up on and exploited by the classifier, resulting in better classification results but not necessarily better alignment results. Therefore, we consider the results across each of the five different versions of the corpus not directly comparable.

\subsection{LM Adaptations}
\label{ssct:lm-adapt}

We use the data and the Roberta engine provided by \citet{pcm_paper_baseline} and \citet{lin2023low} 
to perform CAT on RoBERTa for SimAlign, PFT on multi-lingual BERT for AWESoME and CAFT on T5 for DiscoPrompt.
In our research,  CAT methodology refers to modifying the alignment generated by the \cite{sabet2020simalign} by utilizing \cite{lin2023low} RoBERTa model for generating alignments using the same synthetic parallel data generated with the neural machine translation, and we want to test whether using \cite{lin2023low} Roberta model can generates more informative alignments and hence better dataset for the Implicit Discourse Relation Classification.  Subsequent, to generating the annotated dataset we fine-tuned the  T5 V1.1 model variants following \cite{chan2023discoprompt} approach, as well as finetuned Roberta model \cite{liu2020importance}. The outcomes of this process are detailed in our results section, specifically in Table \ref{tab:simAlignCATAlign_results}.

For the Continual Adaptive Fine-Tuning (CaFT) approach, which we applied across all our generated projected alignment datasets (GizaPy, SimAlign, SimAlign+ CAT,AWESome , AWESome + PFT ), in which we initially leveraged the English PDTB dataset. This involved fine-tuning a T5 v1.1 model on the English PDTB dataset, adhering to the hyperparameters recommended by \cite{chan2023discoprompt}. This model was then subjected to further fine-tuning, a process we refer to as continual adaptive fine-tuning "CaFT", using the NP (Nigerian Pidgin) annotated dataset. The objective of this phase was to ascertain whether the capabilities of larger LLM variants, such as the T5 v1.1 Large, could be leveraged to mitigate the potential overfitting issues that might arise when fine-tuning T5 v1.1 Large from scratch on our projected annotated pdtb data. And we found that CaFT to achieve state-of-the-art results for all the generate dataset, as reported in our results section.


\subsection{Relation Classification}
\label{ssct:relclass}


we focus on \textit{implicit} relations in this paper because this has traditionally been the focus of neural classifiers, allowing us to more easily compare to related work \cite{liu2020importance,chan2023discoprompt}. For the same reason, we use the PDTB 2.0, despite the more recent PDTB 3.0 being available \cite{pdtb3.0}.
Regarding classifier setup, we build on DiscoPrompt \cite{chan2023discoprompt}. We try both systems directly and experiment with different versions of the underlying language models for DiscoPrompt.




In our study, we employed the T5v1.1 model variants as recommended by \cite{chan2023discoprompt} in their work on the state-of-art English Implicit discourse relation classifier DiscoPrompt \cite{chan2023discoprompt}. This included the use of the T5 v1.1 base model to test our hypothesis that a smaller variant might offer better generalization capabilities, especially when trained on purely synthetic data, as it may be less prone to overfitting compared to larger models, in our results \ref{sec:results} we have found continual adaptive fine-tuning DiscoPrompt T5 Large overfits all the generated dataset for the 4-way classification except for the AweSoME aligner generated dataset against zeroshot from state-of-art English implicit discourse relation classification on the Nigerian pidgin, at the same . The T5 v1.1 models vary in size: the small version comprises 60,511,616 parameters, the base version has 222,903,552 parameters, and the large version contains 750,251,008 parameters. \cite{chan2023discoprompt} also performed soft prompt tuning with a prompt learning rate of 0.3. We adhered to their suggestion of limiting the number of soft tokens to 20. As a result, the number of trainable parameters in the Discoprompt are: 546,304 for the T5v1.1 small model, 1,212,672 for the base version, and 2,141,184 for the large variant. For the DiscoPrompt models, we directly fine-tuned the T5 V1.1 model variants on the annotated dataset. In contrast, for the CaFT approach, we initially fine-tuned the T5v1.1 models on the real annotated English PDTB dataset, followed by Continual Adaptive Fine-Tuning (CaFT) on the annotated projected Pidgin dataset. This was done to test our hypothesis that the model, already fine-tuned on English PDTB, would effectively utilize its knowledge about Implicit Discourse Relation Classification when further trained on the NP dataset.



==> tables/MachineTranslation.tex <==
\begin{table*}[h]
\centering
\caption{Model Performance: English to Nigerian Pidgin (En To NP) and Nigerian Pidgin to English (NP to EN)}
\label{tab:model_performance}
\begin{tabular}{|l|c|c|}
\hline
\textbf{Models}    & \textbf{En To NP} & \textbf{NP to EN} \\ \hline
MSP                &                   &       20.078      \\ \hline
MSP Bidirectional  &                   &                   \\ \hline
M2m100             &                   &                   \\ \hline
\cite{lin2023low}  &       36.35       &          34.04     \\ \hline
\end{tabular}
\end{table*}


==> tables/allresults.tex <==
\begin{table*}[!ht]
\centering

\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccc}
\hline
\textbf{Model/Method} & \textbf{4-way f$_{1}$} & \textbf{4-way Accuracy } & \textbf{11-way f$_{1}$} & \textbf{11-way  Accuracy} \\
\hline
\textbf{DP-CAFT T5 Large AWESoME RB} & 0.438 & 0.57 & \textbf{0.345} & 0.475 \\
\textbf{DP-CAFT T5 Large AWESoME+PFT RB} & \textbf{0.441} & 0.55 & 0.343 & 0.466 \\
\textbf{DP-CAFT T5 Large SimAlign RB} & 0.433 & 0.61 & 0.237 & 0.407 \\
\textbf{DP-CAFT T5 Large Simalign+CAT RB} & 0.409 & 0.59 & .226 & 0.403 \\
\textbf{DP-CAFT T5 Large Giza-py RB} & 0.432& 0.552 & 0.298 &0.463 \\
\hdashline
\textbf{\textcolor{red}{DP-CAFT T5 Large AWESoME AB}} & 0.409 & 0.561 & 0.303 & 0.414 \\
\textbf{\textcolor{red}{DP-CAFT T5 Large AWESoME+PFT AB}} & 0.382 & 0.491 & 0.289 & 0.405 \\

\textbf{\textcolor{red}{DP-CAFT T5 Large SimAlign AB}} & 0.367 & 0.498 & 0.300 & 0.409 \\
\textbf{\textcolor{red}{DP-CAFT T5 Large SimAlign+CAT AB}} & 0.362 & 0.502 & 0.254 & 0.396 \\
\textbf{\textcolor{red}{DP-CAFT T5 Large Giza-py AB}} &0.366 & .0531&0.243 &0.362 \\
\hdashline
\textbf{DP-CAFT T5 Base AWESoME RB} & 0.343 & 0.493 & 0.201 & 0.377 \\
\textbf{DP-CAFT T5 Base AWESoME+PFT RB} & 0.381 & 0.536 & 0.239 & 0.398 \\
\textbf{DP-CAFT T5 Base SimAlign RB} & 0.382 & 0.595 & 0.22 & 0.351 \\
\textbf{DP-CAFT T5 Base SimAlign+CAT RB} & 0.352 & 0.559 & 0.232 & 0.371 \\
\textbf{DP-CAFT T5 Base Giza-py RB} & 0.382&\textbf{0.595} &0.220 & 0.351\\
\hdashline
\textbf{\textcolor{red}{DP-CAFT T5 Base AWeSoME AB}} & 0.368 & 0.466 & 0.275 & 0.337 \\
\textbf{\textcolor{red}{DP-CAFT T5 Base AWESoME+PFT AB}} & 0.409 & 0.579 & 0.251 & 0.416 \\
\textbf{\textcolor{red}{DP-CAFT T5 Base SimAlign AB}} & 0.342 & 0.468 & 0.243 & 0.364 \\
\textbf{\textcolor{red}{DP-CAFT T5 Base SimAlign+CAT AB}} & 0.334 & 0.461 & 0.223 & 0.391 \\
\textbf{\textcolor{red}{DP-CAFT T5 Base Giza-py AB}} &0.351 &0.55 & 0.178& 0.281\\
\hline
\hline
%%%%%%%%%%% Scratch Models
%%%Fulltransfer
\textbf{DP T5 Large AWESoME NM} & 0.35 & 0.5035 & 0.239 & 0.40 \\
\textbf{DP T5 Large AWESoME+PFT NM} & 0.369 & 0.5135 & 0.249 & 0.414 \\
\textbf{DP T5 Large SimAlign NM} & 0.296& 0.515 & 0.190 & 0.325 \\
\textbf{DP T5 Large SimAlign+CAT NM} & 0.3306 & 0.450 & 0.177 & 0.364 \\
\textbf{DP T5 Large Giza-py NM} & 0.205& 0.398 & 0.134 &0.321 \\
\hdashline
%%%% AC LARGE
\textbf{\textcolor{red}{DP T5 Large AWESoME AB NM}} &0.217 & 0.411 & 0.124 & 0.309 \\
\textbf{\textcolor{red}{DP T5 Large AWESoME+PFT AB NM}} & 0.133  & 0.321 & 0.095 & 0.316 \\
\textbf{\textcolor{red}{DP T5 Large SimAlign AB NM}} & 0.266 & 0.529 & 0.116 & 0.2601 \\
\textbf{\textcolor{red}{DP T5 Large SimAlign+CAT AB NM}} &0.134 & 0.323 & 0.0966& 0.316 \\
\textbf{\textcolor{red}{DP T5 Large Giza-py AB NM}} &0.124 & 0.3144 & 0.082 &0.31 \\

%%%scratch Base models

\hdashline
%%% Fulltransfer SCRATCH BASE
\textbf{DP T5 Base AWESoME NM} & 0.337 & 0.5 & .26 & 0.38\\
\textbf{DP T5 Base AWESoME+PFT NM} & 0.35 & 0.518 & 0.247 & 0.393 \\
\textbf{DP T5 Base SimAlign NM} & 0.3744 & 0.59 & 0.24 & 0.38 \\
\textbf{DP T5 Base SimAlign+CAT NM} & 0.351 & 0.5588 & .23 & 0.371 \\
\textbf{DP T5 Base Giza-py NM} & 0.3422& 0.477 & 0.267 &0.384\\
\hdashline
%%%AC SCRATCH BASE
\textbf{\textcolor{red}{DP T5 Base AWESoME AB NM}} &0.383 & 0.503 & 0.308 & 0.386 \\
\textbf{\textcolor{red}{DP T5 Base AWESoME+PFT AB NM}} & 0.392  & 0.522 & 0.29 & 0.386 \\
\textbf{\textcolor{red}{DP T5 Base SimAlign AB NM}} & 0.320 & 0.398 & 0.213 & 0.337 \\
\textbf{\textcolor{red}{DP T5 Base SimAlign+CAT AB NM}} &0.1971 & 0.382 &  0.1107& 0.2941 \\
\textbf{\textcolor{red}{DP T5 Base Giza-py AB NM}} & 0.138  & 0.330 & 0.096 &0.319 \\


\hline
\textbf{DP English T5 Large ZeroShot NP} & 0.406 & 0.576 & 0.235 & 0.359 \\
\textbf{DP English T5 Base ZeroShot NP} & 0.349 & 0.581 & 0.172 & 0.307 \\
\textbf{DP T5 Base English ZeroShot Translated } & 0.309&0.43 &0.154 & 0.41\\
\textbf{DP T5 Large English ZeroShot Translated} & 0.408 & 0.5 &0.2 & 0.47\\


\hline
\end{tabular}
\end{adjustbox}
\caption{Comparative Performance Evaluation of Different variants of DiscoPrompt model and training procedures, each using single synthetic dataset (PFT, AweSoME, CaT, SimAlign) (top half of the table) or ZeroShot with the English DiscoPrompt (bottom half of the table). AB = alignment-based, RB = relation-based, DP = DiscoPrompt, CAFT = continual adaptive fine-tuning, CAT = cross-lingual adaptive training, PFT = parallel fine-tuning, NM = Naija model in which we fine-tuned DiscoPrompt Base/Large exclusively on our NP PDTB dataset, and specific alignment strategies such as AweSoME and SimAlign. The metrics are segmented into 4-class and 11-class accuracies and F1 scores to provide a comprehensive view of each model's effectiveness across different categorizations.}
\label{tab:ablation}
\end{table*}


==> tables/baselines.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
model/method        & train & test & 4-way f1 & 4-way acc & 11-way f1 & 11-way acc \\ \hline
DiscoPrompt T5 base & PDTB  &  NP  & 0.349 & 0.581 & 0.172 & 0.307    \\ %\hline
DiscoPrompt T5 large & PDTB  & NP   & 0.406 & 0.576 & 0.235 & 0.359         \\ \hline \hline
DiscoPrompt NP T5 base & NP    & NP   &   0.392       &   0.52        &      0.327      &      0.386      \\ %\hline
DiscoPrompt NP T5 large & NP    & NP   &   0.217      &   0.411       &       0.124   &   0.309        \\ \hline
\end{tabular}
\caption{Baselines: 1) taking DiscoPrompt as is (trained on the English PDTB), testing on NP (TODO: specify in text where this is coming from and how it came to be) and 2) training DiscoPrompt on the NP data and testing on a test section of NP data (TODO: explain in text how we split up the NP data into train/test sections) .}
\label{tab:baselines}
\end{table*}


==> tables/confusionMatrix/AweSoMEPFT_4Way.tex <==
\begin{table}[h!]
    \centering
    \begin{adjustbox}{ width=\columnwidth}
    \begin{tabular}{c|cccc}
    \textbf{True\textbackslash Prediction} & \textbf{Comparison} & \textbf{Contingency} & \textbf{Expansion} & \textbf{Temporal} \\
    \hline
    \textbf{Comparison} & 2 & 0 & 1 & 0 \\
    \textbf{Contingency} & 9 & 80 & 35 & 3 \\
    \textbf{Expansion} & 10 & 105 & 175 & 8 \\
    \textbf{Temporal} & 3 & 20 & 11 & 18 \\
    \end{tabular}
    \end{adjustbox}
    \caption{4-way classification Confusion Matrix for the Naija Model DiscoPrompt T5 Large with CaFT on dataset generated by AweSoME+PFT aligner}
    \label{tab:my_label}
\end{table}



==> tables/extractionExamples.tex <==
% \begin{table*}
%     \centering
%     \begin{tabular}{|>{\RaggedRight}p{2.5cm}|p{4cm}|p{4cm}|p{4cm}|}
%         \hline
%         & Giza-py & SimAlign & AwesomeAlign \\
%         \hline
        
%         Arg1En & Who's telling the truth & & \\
%         \hline
%         Arg2En & Everybody -- and nobody & & \\
%         \hline
%         Arg1PCM & Who dey tell di truth? & & \\
%         \hline
%         Arg2PCM & Everybody nobody. and nobody. & & \\
%         \hline
%     \end{tabular}
%     \caption{PCM Text" Who dey tell di truth? Everybody and nobody." and 
%         En Text "Who's telling the truth? Everybody -- and nobody" Then the extracted Arg1PCM, Arg2PCM as well as the real annotated English Arg1En, Arg2En
%         }
%     \label{tab:alignment_examples}
% \end{table*}

==> tables/resultsAwesomeAlign.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Model & 11-class acc. & 11-class f1 & 4-class acc. & 4-class f1 \\
\hline
CaFT DiscoPrompt T5v1.1 large & 0.404 & 0.246 & 0.519 & \textbf{0.502} \\
CaFT DiscoPrompt T5v1.1 base & 0.400 & \textbf{0.251} & 0.512 & 0.492 \\
DiscoPrompt T5v1.1 large  & 0.243 & 0.047 & 0.424 & 0.186 \\
DiscoPrompt T5v1.1 base & 0.380 & 0.249 & 0.485 & 0.480 \\
DiscoPrompt T5v1.1 small  & 0.276 & 0.101 & 0.391 & 0.323 \\
BMGF-RoBERTa& \textbf{0.418} & 0.244 & 0.570 & 0.391 \\ 
\hdashline
\textcolor{red}{NaijaDiscoRealPidginCaFTBase} & 0.40 & 0.24 & 0.468 &  0.4187 \\
% \textcolor{brown}{NaijaDiscoRealPidginCaFTBase} & 0.40 & 0.24 & 0.468 &  0.4187 \\
\hdashline
\textcolor{blue}{NDRealNP-Data-ENDPBase} & 0.346 & 0.140 & 0.444 &  0.329 \\
\hdashline
\textcolor{green}{TranslatedNaijaUsingEnDPBase} & 0.410 & 0.154 & 0.435 &  0.309 \\
\textcolor{brown}{TranslatedNaijaUsingEnDPLarge} & 0.468 & 0.198 & 0.502 & 0.408\\
\hdashline
Majority vote & 0.263 & 0.109 & \textbf{0.526} & 0.362 \\

\hline
\end{tabular}
\caption{Results on AWESoME}
\label{tab:awesomealing_results}
\end{table*}


==> tables/resultsAwesomeAlignParallelFineTuning.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Model & 11-class acc. & 11-class f1 & 4-class acc. & 4-class f1 \\
\hline

CaFT DiscoPrompt T5v1.1 large  &\textbf{0.431}&0.292&0.553&\textbf{0.537} \\
CaFT DiscoPrompt T5v1.1 base & 0.383 & 0.246 & 0.497 & 0.486 \\


DiscoPrompt T5v1.1 large  & 0.416 & \textbf{0.293} & 0.521 & 0.514 \\
DiscoPrompt T5v1.1 base& 0.372 & 0.244 & 0.502 & 0.478 \\
DiscoPrompt T5v1.1 small  & 0.270 & 0.100 & 0.391 & 0.323 \\

BMGF-RoBERTa & 0.427 & 0.224 & \textbf{0.609} & 0.462 \\
\hdashline
\textcolor{red}{NaijaDiscoRealPidginCaFTBase} & 0.388 & 0.198 & 0.4805 &  0.419 \\
\hdashline
\textcolor{blue}{NaijaDiscoNPDataENDP} & 0.346 & 0.140 & 0.444 &  0.329 \\
\hdashline
\textcolor{green}{TranslatedNaijaUsingEnDPBase} & 0.410 & 0.154 & 0.435 &  0.309 \\
\textcolor{brown}{TranslatedNaijaUsingEnDPLarge} & 0.468 & 0.198 & 0.502 & 0.408\\
\hline
\hdashline
Majority vote & 0.261 & 0.108 & 0.528 &  0.365 \\
\hline
\end{tabular}
\caption{Results on AWESoME+PFT}
\label{tab:awesomealing_pft_results}
\end{table*}


==> tables/resultsCATSimAlign.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Model/Prompt & 11-class acc. & 11-class f1 & 4-class acc. & 4-class f1 \\
\hline
CAT on DiscoPrompt T5v1.1 large & 0.4289 & 0.2768 & 0.5597 & 0.5293 \\
CAT on DiscoPrompt T5v1.1 base & 0.4037 & 0.2595 & 0.5288 & 0.5040 \\
FT5 on simAlign & 0.356 & 0.206 & 0.487 & 0.454 \\
DP T5v1.1 on simAlign & 0.375 & 0.227 & \textbf{0.501} & \textbf{0.476} \\
DP T5v1.1 on simAlign (LR 0.5) & \textbf{0.382} & \textbf{0.253} & \textbf{0.496} & \textbf{0.483} \\
DP T5v1.1 Small on simAlign & 0.372 & 0.219 & 0.479 & 0.466 \\
\hline
\end{tabular}
\caption{Results of SimAlignments method}
\label{tab:simAlign_results}
\end{table*}


==> tables/resultsGizaPy.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Model & 11-class acc. & 11-class f1 & 4-class acc. & 4-class f1 \\
\hline
% DPFT5 on GizaPy & 0.368 & 0.231 & 0.471 & 0.452 \\
CaFT DiscoPrompt T5 T5v1.1 large & 0.404 & \textbf{0.264} & 0.523 & \textbf{0.494} \\

CaFT DiscoPrompt T5 T5v1.1 base & 0.370 & 0.220 & 0.499 & 0.469 \\


DiscoPrompt T5v1.1 large & 0.285 & 0.106 & 0.380 & 0.320 \\
DiscoPrompt T5v1.1 base  & 0.367 & 0.231 & 0.494 & 0.475 \\
% DP T5v1.1 on GizaPy (LR 0.5)& 0.371 & 0.239 & 0.488 & 0.472 \\
DiscoPrompt T5v1.1 small & 0.341 & 0.211 & 0.460 & 0.442 \\
BMGF-RoBERTa & \textbf{0.424} & 0.228 &  \textbf{0.558} &  0.438  \\
\hdashline
\textcolor{red}{NaijaDisco} & 0.426&0.165&0.456&0.342 \\

\textcolor{brown}{TranslatedNaijaUsingEnDPLarge} & 0.468 & 0.198 & 0.502 & 0.408\\
\hdashline
Majority vote & 0.263 & 0.11 & 0.52 & 0.363 \\
\hline
\end{tabular}
\caption{Results on Giza-Py}
%\caption{Results of Different Models/Prompts on GizaPy. DPFT5 stands for Discoprompt on FlanT5, and by default, the prompt learning rate is 0.3, DP stands for Discoprompt}
\label{tab:gizapy_results}
\end{table*}


==> tables/resultsSimAlign.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Model & 11-class acc. & 11-class f1 & 4-class acc. & 4-class f1 \\
\hline
CaFT DiscoPrompt T5v1.1 large & \textbf{0.428} & \textbf{0.276} & 0.559 & \textbf{0.529}\\
CaFT DiscoPrompt T5v1.1 base & 0.403 & 0.259 & 0.528 & 0.504 \\
% DPFT5 on simAlign & 0.356 & 0.206 & 0.487 & 0.454 \\
DiscoPrompt T5v1.1 large &  0.273 & 0.075 & 0.405 & 0.263 \\
DiscoPrompt T5v1.1 base  & 0.375 & 0.227 & 0.501 & 0.476 \\
% DP T5v1.1 on simAlign (LR 0.5) & \textbf{0.382} & \textbf{0.253} & \textbf{0.496} & \textbf{0.483} \\

DiscoPrompt T5v1.1 small & 0.372 & 0.219 & 0.479 & 0.466 \\
BMGF-RoBERTa & 0.413  & 0.206 &  \textbf{0.590} &  0.399  \\
\hdashline
\textcolor{red}{NaijaDiscoRealPidginCaFTBase} & 0.429 & 0.204 & 0.471 &  0.3826 \\
\hdashline
\textcolor{blue}{NaijaDiscoNPDataENDP} & 0.346 & 0.140 & 0.444 &  0.329 \\
\hdashline
\textcolor{green}{TranslatedNaijaUsingEnDPBase} & 0.410 & 0.154 & 0.435 &  0.309 \\
\textcolor{brown}{TranslatedNaijaUsingEnDPLarge} & 0.468 & 0.198 & 0.502 & 0.408\\
\hdashline
Majority vote & 0.265 & 0.111 & 0.525 & 0.361 \\

% \hdashline
% CaFT+CaTAlign DPT5v1.1 Base & 03877 & 0.25 & 0.51 & .488  \\

% CaFT+CaTAlign DPT5v1.1 large & - & - & - & - \\ 
% BMGF Roberta (best f1 epoch) & - & - &  = &  -  \\

\hline
\end{tabular}
\caption{Results on SimAlign}
\label{tab:simAlign_results}
\end{table*}


==> tables/resultsSimAlignRobertaPCM.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Model & 11-class acc. & 11-class f1 & 4-class acc. & 4-class f1 \\
\hline

CaFT on DiscoPrompt T5v1.1 large & \textbf{0.416} & \textbf{0.277} & \textbf{0.529} & \textbf{0.512} \\
CaFT DiscoPrompt T5v1.1 base & 0.387 & 0.250 & 0.510 & 0.488  \\
DiscoPrompt T5v1.1 large &  0.286 & 0.116 & 0.405 & 0.377\\
DiscoPrompt T5v1.1 base  & 0.290 & 0.156 & 0.415 & 0.401 \\
DiscoPrompt T5v1.1 small & 0.273 & 0.106 & 0.415 &  0.345 \\
BMGF-RoBERTa (batch=16) & - & - &  0.562 &  0.298 \\

\hdashline
\textcolor{red}{NaijaDiscoRealPidginCaFTBase} & 0.44 & 0.179 & 0.48 &  0.365 \\

\hdashline
\textcolor{blue}{NaijaDiscoNPDataENDP} & 0.346 & 0.140 & 0.444 &  0.329 \\
\hdashline
\textcolor{green}{TranslatedNaijaUsingEnDPBase} & 0.410 & 0.154 & 0.435 &  0.309 \\
\textcolor{brown}{TranslatedNaijaUsingEnDPLarge} & 0.468 & 0.198 & 0.502 & 0.408\\
\hdashline
Majority vote & 0.264 & 0.111 & 0.524 & 0.360 \\
\hline
\end{tabular}
\caption{Results on SimAlign+CAT}
\label{tab:simAlignCATAlign_results}
\end{table*}

